Fast and simple inner-loop algorithms of static / dynamic BLP estimations

This study investigates computationally efficient inner-loop algorithms for estimating static/dynamic BLP models. It provides the following ideas for reducing the number of inner-loop iterations: (1). Add a term relating to the outside option share in the BLP contraction mapping; (2). Analytically represent the mean product utilities as a function of value functions and solve for value functions (for dynamic BLP); (3). Combine an acceleration method of fixed-point iterations, especially the Anderson acceleration. They are independent and easy to implement. This study shows the good performance of these methods using numerical experiments.

==> introduction.tex <==
Demand estimation is the basis of many economic analyses. The estimation method based on the random coefficient logit model proposed by \citet{berry1995automobile} (henceforth BLP) has been widely applied in the literature. Though \citet{berry1995automobile} initially considered a static demand model, The model and estimation procedure have been extended to dynamic demand models, such as durable goods and goods with switching costs (e.g., \citealp{gowrisankaran2012dynamics}; \citealp{shcherbakov2016measuring}). The models are known as dynamic BLP. In these models, products' mean utilities $\delta$ are numerically solved in the inner loop, and econometricians search for the parameter values minimizing the GMM objective in the outer loop. 

Nevertheless, one obstacle to the method is the computational time. The computational burden can be high because of the need to repeat fixed-point iterations in the inner loop, especially when we consider estimations of complicated demand models or estimations with large datasets. This study investigates computationally efficient inner-loop algorithms for estimating static and dynamic BLP models. Computationally efficient inner-loop algorithms for estimating static BLP models have been intensively investigated in the literature, including \citet{kalouptsidi2012market}, \citet{reynaerts2012enhencing}, \citet{conlon2020best}, \citet{pal2023comparing}. Nevertheless, I show there is further room for improvement even in static BLP models, let alone dynamic BLP models. 

Regarding static BLP models, I newly introduce a new fixed-point iteration mapping $\delta^{(n+1)}=\delta^{(n)}+\left(\log\left(S_{j}^{(data)}\right)-\log\left(s_{j}(\delta^{(n)})\right)\right)-\left(\log\left(S_{0}^{(data)}\right)-\log\left(s_{0}(\delta^{(n)})\right)\right)$, by slightly modifying the traditional BLP contraction mapping $\delta^{(n+1)}=\delta^{(n)}+\left(\log\left(S_{j}^{(data)}\right)-\log\left(s_{j}(\delta^{(n)})\right)\right)$.\footnote{$S_{jt}^{(data)}$ denotes product $j$'s observed market share, and $s_{j}(\delta)$ denotes the market share predicted by the structural model.} The difference with the traditional BLP contraction mapping is the term $\log\left(S_{0}^{(data)}\right)-\log\left(s_{0}(\delta^{(n)})\right)$, and it is straightforward to code in any programming languages. When there is no consumer heterogeneity, applying the new mapping immediately converges to the solution after one iteration for any initial values of $\delta$. Though there is no guarantee that the mapping is a contraction, this study finds that it converges and reduces the number of iterations in the Monte Carlo simulation settings experimented in the previous studies (\citealp{dube2012improving}; \citealp{lee2015computationally}) and \citet{nevo2001measuring} and Berry et al. \citeyearpar{berry1995automobile,berry1999voluntary}'s dataset. Note that the speed-up is prominent, especially when the size of consumer heterogeneity is relatively small.

The current study also compares the performance of some acceleration methods of fixed-point iterations (Anderson acceleration, Spectral, SQUAREM), and it finds that Anderson acceleration, which has not been paid much attention to in the literature \footnote{\citet{duch2023evaluating} is the exception. As discussed in the online appendix of their paper, they applied the stabilized version of the Anderson acceleration method proposed by \citet{zhang2020globally} to estimate a random coefficient nested logit model with a large nest parameter.} \footnote{\citet{conlon2020best} pointed out in footnote 81 of their paper that ``Anderson acceleration'' using ``anderson'' function in Python Scipy package was too slow and unreliable to be worth considering. I could verify it by using PyBLP. However, the ``Anderson acceleration'' method in Python Scipy package is aimed at solving general nonlinear equations, and the algorithm is not the same as the ``Anderson acceleration'' for fixed point iterations discussed in the current paper.}, performs better than the others, and contributes to further reductions in the number of iterations and computation time. The strategy works even when the size of consumer heterogeneity is large. Because we can easily code the new mapping by adding a few lines when we use the traditional BLP contraction mapping, the current study recommends coding the new mapping first, and then consider combining the acceleration of fixed point iterations, especially Anderson acceleration, if necessary. Note that Anderson acceleration method is intuitive, and it is also relatively easy to code.

Regarding dynamic BLP models, I propose to analytically represent mean product utility $\delta$ as a function of value function $V$, solve for $V$ by applying a mapping of $V$, and recover $\delta$ using the analytical formula and the values of $V$. Note that the previous studies (e.g., \citealp{gowrisankaran2012dynamics}) have applied an inner loop algorithm essentially consisted of solving for two types of variables $\delta$ and $V$. In the current algorithm, we only have to solve for only one type of variable $V$, and it leads to reducing the number of iterations in the inner loop. When we further combine the acceleration method of fixed point iterations, especially Anderson acceleration, we can further reduce the number of iterations.

Note that the acceleration methods of fixed point iterations are useful not only for the inner-loop algorithms of static/dynamic BLP estimations, but also for efficiently solving any types of fixed-point problems, including dynamic models with value functions and supply-side pricing equilibrium. Built-in packages of the acceleration methods, including Anderson acceleration, Spectral, and SQUAREM, are available in some programming languages. Even when unavailable, they are easy to code because of their simple formulas. Hence, being accustomed to using such built-in packages or coding the functions to implement the acceleration methods tailoring practitioners' needs would be useful.


We should keep in mind that the performance of acceleration methods largely relies on the types of fixed-point problems, as discussed in \citet{tang2023accelerating}, comparing several acceleration methods including Anderson and SQUAREM\footnote{\citet{tang2023accelerating} did not compare the performance of the spectral algorithm.} in the context of statistics applications. For instance, Anderson performs better than SQUAREM in some models, but worse than SQUAREM in other models. Though the current study finds that the Anderson acceleration performs fairly well and outperforms the others in most of the static and dynamic BLP models\footnote{As shown in Appendix \ref{subsec:large_hetero}, the current study finds that the Anderson acceleration fails in an artificial setting where the size of consumer heterogeneity is too large. Even in the setting, the spectral and SQUAREM algorithms successfully converge.}, the spectral and SQUAREM algorithms work much better than the original fixed point iterations. Hence, though the current study recommends using Anderson acceleration, the spectral and SQUAREM algorithms can be good alternatives, and worth trying in case Anderson does not work well. Note that when we apply the spectral or SQUAREM algorithm, we should be careful about the choice of step sizes $\alpha$, though not paid much attention to in the previous economics literature. When we do not use appropriate step sizes, the algorithms can lead to divergence. We briefly discuss it in Section \ref{sec:Acceleration-methods}.


This study contributes to the literature by mainly providing the following ideas or insights to reduce the number of inner-loop iterations in the static/dynamic BLP estimations: (1). New mapping $\delta^{(n+1)}=\delta^{(n)}+\left(\log\left(S_{j}^{(data)}\right)-\log\left(s_{j}(\delta^{(n)})\right)\right)-\left(\log\left(S_{0}^{(data)}\right)-\log\left(s_{0}(\delta^{(n)})\right)\right)$; (2). Analytically represent mean product utilities $\delta$ as a function of value functions $V$ and solve for $V$ (for dynamic BLP models); (3). Combine the acceleration method of fixed point iterations, especially Anderson acceleration. These methods are independent, and relatively easy to implement. Practitioners can implement some or all of them when they face difficulties in the computational burden.\footnote{\citet{fukasawa2024lightbulb} applies some of these ideas to the dynamic demand estimation of the light bulb market by specifying a durable goods model with forward-looking consumers and replacement demand. The computation time is reduced by more than 10 times with these strategies. Without them, the expected estimation time would be more than 10 hours. }

The rest of this article is organized as follows. Section \ref{sec:Literature} discusses the relations to the previous studies. In Section \ref{sec:Static-BLP-model}, we discuss inner-loop algorithms for estimating static BLP models. In Section \ref{sec:Dynamic-BLP-model}, we discuss inner-loop algorithms for estimating dynamic BLP models. Readers interested only in the static BLP models can skip the section. Section \ref{sec:Acceleration-methods} discusses the acceleration methods of fixed point iterations, including Anderson acceleration, spectral, and  SQUAREM. Note that the discussion in the section applies to any fixed-point iteration. Section \ref{sec:Numerical-Experiments} shows the results of numerical experiments on static/dynamic BLP models. Section \ref{sec:Conclusion} concludes.

Appendix \ref{sec:Additional-results} shows additional results and discussions. In Appendix \ref{sec:DDC}, we discuss that the idea of the proposed inner-loop algorithm for estimating dynamic BLP models can be used in estimating dynamic discrete choice models with unobserved payoffs, which have been considered in \citet{kalouptsidi2020linear} and others. Appendix \ref{sec:Proof} shows all the proofs of the mathematical statements.


